Learning, Computing, and Trustworthiness in Intelligent IoT Environments: Performance-Energy Tradeoffs

An Intelligent IoT Environment (iIoTe) is comprised of heterogeneous devices that can collaboratively execute semi-autonomous IoT applications, examples of which include highly automated manufacturing cells or autonomously interacting harvesting machines. Energy efficiency is key in such edge environments, since they are often based on an infrastructure that consists of wireless and battery-run devices, e.g., e-tractors, drones, Automated Guided Vehicle (AGV)s and robots. The total energy consumption draws contributions from multipleiIoTe technologies that enable edge computing and communication, distributed learning, as well as distributed ledgers and smart contracts. This paper provides a state-of-the-art overview of these technologies and illustrates their functionality and performance, with special attention to the tradeoff among resources, latency, privacy and energy consumption. Finally, the paper provides a vision for integrating these enabling technologies in energy-efficient iIoTe and a roadmap to address the open research challenges

==> 3-use-cases.tex <==

\section{Intelligent IoT environments: the manufacturing plant example} \label{sec:use_cases}


The use case in Fig. \ref{fig:manufacturing} describes an example of machine to machine collaboration in an industrial plant. The scene starts with a customer (the end-user) of a shared manufacturing plant ordering a product by specifying a manufacturing goal via step (1). In step (2), a machine orchestration and associated process plan is determined to manufacture the desired product. The event-based process planner is responsible of observing the manufacturing process and reacting when the health state of a concerned machine changes. For example, by re-scheduling a given task in a non-responding machine. In step (3), a robot or AGV is tasked to transport the work-piece to the next production step and  manufacturing process data is sent to involved machines. As these machines may be operated by the plant owner or a third-party operator, contractual arrangements need to be set up, for which a distributed ledger is used. Further, comprehensive security mechanisms are applied to ensure privacy and security of customer data. In step (4), a local AI on board of the robot decides how the robot picks a work-piece and places it in the next machine. From the handling of the work piece, local AI on the robot re-trains itself, and federates the learned process parameters to other robots through model update on the Edge (5). 

\begin{figure}[!ht]
\centering
\includegraphics[width=4in]{figures/uc3_TGCN.pdf}
\caption{IntellIoT-enabled NG \gls{iot} manufacturing use case.}
\label{fig:manufacturing}
\end{figure}


%If the confidence-level of the local AI is low and it cannot pick and place the workpiece safely, it again can request support from a human plant operator or machine owner as shown in step (6). Utilizing AR/VR technologies, the human can virtually grab the workpiece to support the robot. A tactile communication needs to be established for this interaction, under consideration of security and privacy. Additionally, 3D cameras can be used to generate an accurate enough reconstruction of the surroundings and the robot itself which allows the full control and visual information about the parameters of the robot. For grabbing and haptic feedback to the user, special user input devices (e.g., a stylus or glove) need to be developed. If support from a remote operator is needed, a tactile communication may not be possible through long-distance internet connection. Hence, the operator would be able to control a virtual robot (overlaying the scanned model with the CAD model), rendered in the local edge, with delayed movement of the real robot. This goes beyond the state-of-art as the supported communication services have very different requirements and can be addressed by relying on the \emph{platform approach} of 5G: NR URLL for the control in downlink, NR eMBB for VR/AR streaming, and Cellular IoT mMTC on the uplink, jointly optimized by a URLL 5G edge server, combined with wired TSN communication through the robot itself. 


%\subsection{Intelligent agricultural fleet }

%Fig. \ref{fig:agriculture} describes an exemplary use case of semi-autonomous vehicle fleet interaction, which will be a common scenario in the future also in other domains (e.g., autonomous cars in traffic or AGVs in industrial plants). This use case entails the provision of new functionalities (e.g., AI algorithm implementations) for \gls{iot} applications by technology providers (e.g. tractor manufacturers) via step (1). A human operator (Farmer or Agriculture fleet management) specifies a goal for autonomous activities (e.g., ploughing or spraying a certain farm field) of the tractor on an Edge infrastructure as depicted in step (2). From the defined goal, a plan for \gls{iot} application instantiation is derived and a deployment of the required functions to the involved devices, e.g., tractor or drones  shown in step (3), is triggered and communicated using the available 5G infrastructure. Next, the deployed AI operates the involved vehicles, which includes dealing with blockages or other adversarial events using sensors of the vehicle (e.g., cameras or LIDAR) via step (4). This can be facilitated by sensing the environment from multiple neighbouring vehicles to collectively train their models and identify objects in a faster and more robust manner. The sensed data can also serve as a training dataset for continually improving the underlying AI models by leveraging e.g., federated/meta learning across vehicles. 

%\begin{figure}[!ht]
%\centering
%\includegraphics[width=4in]{figures/uc1_TGCN.pdf}
%\caption{IntellIoT-enabled NG IoT agriculture use case. 
%}
%\label{fig:agriculture}
%\end{figure}

%Based on the local experience, the vehicle can refine its AI models by continually learning shown by step (4) how to overcome the found obstacles in the future in addition to potentially sharing the learned model with other vehicles.

%In the future, it will also be a common business model for service providers to offer such semi-autonomous vehicles (e.g., to provide farming services). Then, contractual agreements need to be set up using distributed ledger and smart contracts. E.g., ownership of the farmer’s land needs to be confirmed, after which an authorization token is granted along with coordinates of the field. This information will constitute a digital evidence that the field owner authorized the requested services and the area in which the smart equipment operates. Storing performed agricultural activities back in the DLT as historic evidence via step (5) can then be exploited by business models for ecological agriculture and supply chains. Finally, such use cases of vehicle fleet operations will leverage drones to support the fleet management. Then, reliable interaction (e.g., based on 5G NR)  need to take place between the tractor and drone. Drones can be enabled to provide additional data (e.g., video stream) to the vehicle to support its autonomous operation. Further, drones can act as relays and range extender of the 5G infrastructure.
